Reversible Fault-Tolerant Logic

It is now widely accepted that the CMOS technology implementing irreversible logic will hit a scaling limit beyond 2016, and that the increased power dissipation is a major limiting factor. Reversible computing can potentially require arbitrarily small amounts of energy. Recently several nano-scale devices which have the potential to scale, and which naturally perform reversible logic, have emerged. This paper addresses several fundamental issues that need to be addressed before any nano-scale reversible computing systems can be realized, including reliability and performance trade-offs and architecture optimization. Many nano-scale devices will be limited to only near neighbor interactions, requiring careful optimization of circuits. We provide efficient fault-tolerant (FT) circuits when restricted to both 2D and 1D. Finally, we compute bounds on the entropy (and hence, heat) generated by our FT circuits and provide quantitative estimates on how large can we make our circuits before we lose any advantage over irreversible computing.

==> figs/xyqcirc.tex <==
%
% File:   xyqcirc.tex
% Date:   14-Mar-04
% Author: I. Chuang <ichuang@mit.edu>
%
% Definitions for producing quantum circuits with XYPIC in latex
%
% $Log: xyqcirc.tex,v $
% Revision 1.17  2004/03/25 05:01:23  ike
% discard and slash
%
% Revision 1.16  2004/03/25 04:58:42  ike
% added discard, and variable width dmeter
%
% Revision 1.15  2004/03/24 23:43:33  ike
% \dmeter and \sq
%
% Revision 1.14  2004/03/24 20:29:40  ike
% added \t for swap
%
% Revision 1.13  2004/03/24 17:52:16  ike
% removed \w from \gspace
%
% Revision 1.12  2004/03/24 16:38:34  ike
% added small space before |0> for \z
%
% Revision 1.11  2004/03/24 16:23:11  ike
% added \z
%
% Revision 1.10  2004/03/24 16:19:11  ike
% added multiple qubit operations
%
% Revision 1.9  2004/03/24 03:03:44  ike
% typo
%
% Revision 1.8  2004/03/24 02:50:09  ike
% added qv
%
% Revision 1.7  2004/03/24 00:07:34  ike
% add \m matrix op
%
% Revision 1.6  2004/03/23 23:13:10  ike
% misc
%
% Revision 1.5  2004/03/23 23:12:42  ike
% works now
%
% Revision 1.4  2004/03/23 22:22:34  ike
% ifthen also failes - because xymatrix entries in \save...\restore
%
% Revision 1.3  2004/03/23 21:34:36  ike
% no q/c wire switching
%
% Revision 1.2  2004/03/23 21:25:29  ike
% classical qo quantum wire switching try
%
% Revision 1.1  2004/03/23 21:01:46  ike
% Initial revision
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preliminaries

\usepackage{graphicx}

\usepackage[frame,line,arrow,matrix,tips]{xy}	% all that is usually necessary
\CompilePrefix{xygui-}
\makeindex
\pagestyle{empty}

\setlength{\oddsidemargin}{-0.5in}	% 1.25in left margin 
\setlength{\evensidemargin}{-0.5in}	% 1.25in left margin (even pages)

\setlength{\topmargin}{0.0in}		% 1in top margin
\setlength{\textwidth}{6.25in}		% 6.0in text - 1.25in rt margin
\setlength{\textheight}{8.6in}		% Body ht for 1in margins
\addtolength{\topmargin}{-\headheight}	% No header, so compensate
\addtolength{\topmargin}{-\headsep}	% for header height and separation

\begin{document}

\thispagestyle{empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% wires

\def\w{\ar@{-}[l]}
\def\W{\ar@{=}[l]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% labels

% simple label
\def\A#1{\save []="#1" \restore}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% single qubit operations

\def\op#1{*+[F]{\rule[-0.2ex]{0ex}{2.1ex}#1}}	% operator in box
\def\b{*={\bullet}}
\def\o{*={\oplus}}
\def\t{*={\times}}				% for swap gate
\def\sq{*=<6pt,6pt>[F]{}}			% square, for controlled-phase
\def\m#1{\left[\matrix{#1}\right]}		% matrix shortcut
\def\z{*+[]{\rule[-0.2ex]{0ex}{2.1ex}~|0\>}}	% re-init to |0>
\def\discard{*[]{\rule[-0.2ex]{0.75pt}{2.1ex}~}}	% vertical ``|''
\def\slash{*={/}}				% slash for wire bundles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% nop's

\def\N{*-{}\W}
\def\n{*-{}\w}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% misc definitions

\def\>{\rangle}
\def\<{\langle}
\def\ua{\uparrow}

% measurement box
\def\meter{*+[]{\put(-3,0){\includegraphics[scale=.5]{meter.epsf}}~~~~}%
		\ar@{-}[l]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% qubit names (and also revert to qubit wires, vs, cbit wires)

\def\q#1{*+{\rule[-0.2ex]{0ex}{2.1ex}|#1\>}}
\def\qv#1#2{*+{\rule[-0.2ex]{0ex}{2.1ex}|#1\>=|#2\>}}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% multiple qubit gates

% utulity text box for figuring out width of things
\newbox{\sbox}

% empty space of width determined by the text argument
\def\gspace#1{*+{\rule[-0.2ex]{0ex}{2.1ex}%
	\setbox\sbox=\hbox{$#1$}%
	\hspace*{\wd\sbox}}}
	
% n-qubit operation #1=box label, #2=number of qubits (eg d=2 qubits, ddd=4)
\def\gnqubit#1#2{\gspace{#1}
		 \save [].[#2]!C="qq"*[F]\frm{}\restore
		 \save "qq"*[]{#1} \restore}

% two-qubit operation
\def\gtwo#1{\gnqubit{#1}{d}}

% two-qubit operation
\def\gthree#1{\gnqubit{#1}{dd}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ``D'' style measurement gate a-la-cleve, at Michael Nielsen's request

\def\dmeterwide#1#2{*{\xy <0pt,-8pt>;<0pt,8pt> **@{-};
		    <0pt,-8pt>;<#2,-8pt> **@{-} ;
		    <0pt, 8pt>;<#2, 8pt> **@{-} ;
		    <#2,0pt>-<5pt,0pt>*{#1} ;
		    <#2,0pt>*\cir<8pt>{r_l}\endxy}}

\def\dmeter#1{\dmeterwide{#1}{12pt}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

